On Repetitive Finite Automata with Translucent Words

We introduce and study the repetitive variants of the deterministic and the nondeterministic finite automaton with translucent words (DFAwtw and NFAwtw). On seeing the right sentinel, a repetitive NFAwtw need not halt immediately, accepting or rejecting, but it may change into another state and continue with its computation. We establish that a repetitive DFAwtw already accepts a language that is not even semi-linear, which shows that the property of being repetitive increases the expressive capacity of the DFAwtw and the NFAwtw considerably.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{N. Moreira and L. Prigioniero (Eds.): 15th International Workshop on\\ Non-Classical Models of Automata and Applications (NCMA 2025).\\
EPTCS 422, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.422.5}{10.4204/EPTCS.422.5}}
\pdfoutput=1

